MetaV: A Meta-Verifier Approach to Task-Agnostic Model Fingerprinting

For model piracy forensics, previous model fingerprinting schemes are commonly based on adversarial examples constructed for the owner's model as the \textit{fingerprint}, and verify whether a suspect model is indeed pirated from the original model by matching the behavioral pattern on the fingerprint examples between one another. However, these methods heavily rely on the characteristics of classification tasks which inhibits their application to more general scenarios. To address this issue, we present MetaV, the first task-agnostic model fingerprinting framework which enables fingerprinting on a much wider range of DNNs independent from the downstream learning task, and exhibits strong robustness against a variety of ownership obfuscation techniques. Specifically, we generalize previous schemes into two critical design components in MetaV: the \textit{adaptive fingerprint} and the \textit{meta-verifier}, which are jointly optimized such that the meta-verifier learns to determine whether a suspect model is stolen based on the concatenated outputs of the suspect model on the adaptive fingerprint. As a key of being task-agnostic, the full process makes no assumption on the model internals in the ensemble only if they have the same input and output dimensions. Spanning classification, regression and generative modeling, extensive experimental results validate the substantially improved performance of MetaV over the state-of-the-art fingerprinting schemes and demonstrate the enhanced generality of MetaV for providing task-agnostic fingerprinting. For example, on fingerprinting ResNet-18 trained for skin cancer diagnosis, MetaV achieves simultaneously $100\%$ true positives and $100\%$ true negatives on a diverse test set of $70$ suspect models, achieving an about $220\%$ relative improvement in ARUC in comparison to the optimal baseline.

==> tex/app.tex <==
\setcounter{figure}{0}
\renewcommand\thefigure{\Alph{section}\arabic{figure}}    
\setcounter{table}{0}
\renewcommand\thetable{\Alph{section}\arabic{table}}    
\section{Datasets and Target Models}
\noindent\textbf{(1) Skin Cancer Diagnosis} (\textit{abbrev.} \textbf{Skin}). The first scenario covers the usage of deep convolutional neural network (CNN) for skin cancer diagnosis. According to \cite{Yang2020MedMNISTCD}, we train a ResNet-18 \cite{He2016DeepRL} as the target model on DermaMNIST \cite{Yang2020MedMNISTCD}, which consists of $10005$ multi-source dermatoscopic images of common pigmented skin lesions imaging dataset. The input size is originally $3\times{28}\times{28}$, which is upsampled to be $3\times{224}\times{224}$ to fit the input shape of a standard ResNet-18 architecture implemented in torchvision \footnote{\url{https://pytorch.org/vision/stable/_modules/torchvision/models/resnet.html\#resnet18}}. The task is a $7$-class classification task. 

\noindent\textbf{(2) Warfarin Dose Prediction} (\textit{abbrev.} \textbf{Warfarin}). The second scenario covers the usage of FCN for warfarin dose prediction, which is a safety-critical regression task that helps predict the proper individualised warfarin dosing according to the demographic and physiological record of the patients (e.g., weight, age and genetics). We use the International Warfarin Pharmacogenetics Consortium (IWPC) dataset \cite{WhirlCarrillo2012PharmacogenomicsKF}, which is a public dataset composed of $31$-dimensional features of $6256$ patients and is widely used for researches in automated warfarin dosing. According to \citet{Truda2019WarfarinDE}, we use a three-layer multi-layer perception (MLP) with ReLU as the target model, with its hidden layer composed of $100$ neurons. As a notation, we denote the architecture as $(31$-$100$-$1)$. The target model learns to predict the value of proper warfarin dosing, which is a non-negative real-valued scalar with its value in $(0, 300.0]$.

\noindent\textbf{(3) Fashion Generation} (\textit{abbrev.} \textbf{Fashion}) The final scenario covers the usage of FCN for generative modeling. We choose \cite{Xiao2017FashionMNISTAN}, which consists of $60000$  images for articles of clothing of size $28\times{28}$. We train a DCGAN-like architecture \cite{Radford2016UnsupervisedRL} for generative modeling on this task. We solely view the generator as the target model, as a well-trained generator represents more the IP of the model owner because it can be directly used to generate realistic images without the aid of the discriminator. The detailed DCGAN architecture we use is demonstrated in Table \ref{tab:app:dcgan}.


%%%% BEGIN OF DCGAN Table
\input{tex/table/dcgan}
%%%% END OF DCGAN Table

%%% FIG APP
\begin{figure*}[h]
\begin{center}
\includegraphics[width=1.0\textwidth]{img/skin_ru_suite.pdf}
\caption{Curves of robustness and uniqueness of UTAF on Warfarin and Fashion, where the ARUC is reported in the figure title, corresponding to the results in Fig. 2.}
\label{fig:aruc_fps_suite}
\end{center}
\end{figure*}



%%% BEGIN OF MODEL STAT TABLE
\input{tex/table/model_stat}
%%% END OF MODEL STAT TABLE 



%%% BEGIN OF negative suspect model for GAN
\input{tex/table/fcn_gan.tex}
%%% END OF negative suspect models for DCGAN


\section{Details of Suspect Models} We list the composition of the suspect models for all the three scenarios in Table \ref{tab:app:model_stat}. For convenience, we use the following abbreviation: fine-tuning the last layer (=\textit{FTLL}), fine-tuning all layers (=\textit{FTAL}), retraining the last layer (=\textit{RTAL}), retraining all layers (=\textit{RTAL}), weight-pruning (=\textit{WP}), filter-pruning (=\textit{FP}). For constructing distillation-based positive suspect models and independently trained negative suspect models, we implement $3$-$5$ models of diverse architectures and incremental sizes for each of the three target models. For convenience, we index these models as \textit{S, M, L, XL, XLL}. Specifically, these models are:
\begin{itemize}
    \item \textbf{Skin}: \textit{S}=SqueezeNet-1\_0 \cite{Iandola2016SqueezeNetAA}; \textit{M}=ResNet-18 (\citet{He2016DeepRL}, the same as the target model); \textit{L}=DenseNet-161 \cite{Huang2017DenselyCC}; \textit{XL}=AlexNet \cite{Krizhevsky2014OneWT}; \textit{XXL}=VGG-16 \cite{Simonyan2015VeryDC}.
    \item \textbf{Warfarin}: \textit{S}=$(31$-$100$-$1)$ (the same as the target model); \textit{M}=$(31$-$100$-$100$-$1)$; \textit{L}=$(31$-$100$-$100$-$100$-$1)$.
    \item \textbf{Fashion}: \textit{S}=Architecture in Table \ref{tab:app:fcn_gan} with $L=1$; \textit{M}=with $L=2$; \textit{L}=with $L=3$; \textit{XL}=the same as the target model in Table \ref{tab:app:dcgan}. 
\end{itemize}

\section{More Implementation Details.} 
\subsubsection{Hyperparameter Setups.} With no further specifications, we always set the number of fingerprint examples, i.e., $N$, for UTAF and the baselines as $100$ for fair comparisons. We set the learning rate in Algorithm 1 as $0.001$ and the number of iteration as $1000$. In all the three scenarios, we implement the meta-verifier $\mathcal{V}$ as a three-layer fully-connected neural network with the ReLU hidden layer size of $100$.

\subsubsection{Experimental Environment.} All the defenses and experiments are implemented with PyTorch \cite{Paszke2019PyTorchAI}, an open-source software framework for numeric computation and deep learning. All our experiments are conducted on a Linux server running Ubuntu 16.04, one AMD Ryzen Threadripper 2990WX 32-core processor and 2 NVIDIA GTX RTX2080 GPUs.



==> tex/opheline.tex <==
 possibly adopted by the attacker
 
 %%% FIG 5
% \begin{figure}[ht]
% \begin{center}
% \includegraphics[width=0.5\textwidth]{img/war_fa_aruc_fps.pdf}
% \caption{The curves of ARUC when the number of fingerprint examples increases on Warfarin and Fashion.}
% \label{fig:war_fa_aruc_fps}
% \end{center}
% \end{figure}



\begin{itemize}
    \item \textbf{Limited to Classification Tasks.} For fingerprint construction and verification, previous fingerprinting schemes commonly rely on concepts like adversarial examples and classification boundary, which have no direct counterparts in other learning tasks (e.g., regression and generative modeling). As a result, existing fingerprinting schemes could hardly be applied to other important application domains except for classification. 
    \item \textbf{Required Access to Training Data.} To generate adversarial examples as fingerprints for the target model, most existing fingerprinting schemes usually require the access to a set of normal samples from the training data. However, in practical situations, when the training data contains sensitive information or is annotated with huge manual efforts, the model owner is not allowed or unwilling to share the raw data for the fingerprinting process.  
\end{itemize}

Both types of suspect models can be prepared with the aid of public data , with irrelevant public models freely available online, or in cooperation with the model owner to meet the data isolation constraints. 

we do not allow the verifier to access the training data considering the data confidentiality. Instead, we assume the verifier would collaborate with the model owner and request him/her to provide a moderate number of small-scale DNNs trained from scratch on the training data. Besides, 

In this section, we present our detailed design of Universal Task-Agnostic Fingerprinting (UTAF). Below, we first introduce the general pipeline of UTAF.

\begin{itemize}
    \item For an arbitrary model $M_{+} \in \mathcal{M}_{+} \cup \{F\}$, the corresponding sub-objective writes 
    \begin{equation}
        \text{arg}\max_{\mathcal{X}_F, \mathcal{V}}\max(p_{+}(M_+) - p_{-}(M_+) - \delta, 0) := \mathcal{L}_{+}(M_{+}).
    \label{eq:loss_pos}
    \end{equation}
    
   \item For an arbitrary model $M_{-} \in \mathcal{M}_{-}$, the corresponding sub-objective writes
    \begin{equation}
        \text{arg}\max_{\mathcal{X}_F, \mathcal{V}}\max(p_{-}(M_-) - p_{+}(M_-) - \delta, 0) := \mathcal{L}_{-}(M_{-})
        \label{eq:loss_neg},
    \end{equation}
\end{itemize}
where $(p_{-}(M), p_{+}(M)) = \mathcal{V}(M(x_F^{1}) \oplus \hdots \oplus M(x_F^{N}))$, the prediction from the meta-verifier on the concatenated output of a model under test on the adaptive fingerprint. It is worth to notice, we use the ranking loss form in (\ref{eq:loss_pos}) \& (\ref{eq:loss_neg}) with $\delta$ the margin. Combining the two sub-objectives above, we summarize the full learning objective during UTAF's fingerprint construction stage as 

which,

 We consider two types of model compression schemes, i.e., weight pruning (WP) \cite{Han2015LearningBW} and filter pruning (FP) \cite{Li2017PruningFF}.
 
 
 % With more computing power and well-annotated data devoted to building deep neural networks (DNN), corporations as the model owner become aware of the protection of well-trained DNNs as an inseparable part of their intellectual property (IP). However, even with careful access control, the model can be stolen via system or algorithmic attacks (i.e., \textit{model piracy}), strongly violating the IP of the model owner. To obtain evidence on model piracy in the wild, a line of \textit{model fingerprinting algorithms}, which commonly relies on a special set of adversarial examples constructed for the owner's model as the \textit{fingerprints} and verify whether a suspect model is indeed stolen from the original model by matching the behavioral pattern on the fingerprints with one another, are recently proposed. However, these methods are limited to classification models and heavily rely on training data for fingerprint construction, less desirable if the model owner is not allowed or unwilling to share the raw data for fingerprinting.     
